Global Textual Relation Embedding for Relational Understanding

Pre-trained embeddings such as word embeddings and sentence embeddings are fundamental tools facilitating a wide range of downstream NLP tasks. In this work, we investigate how to learn a general-purpose embedding of textual relations, defined as the shortest dependency path between entities. Textual relation embedding provides a level of knowledge between word/phrase level and sentence level, and we show that it can facilitate downstream tasks requiring relational understanding of the text. To learn such an embedding, we create the largest distant supervision dataset by linking the entire English ClueWeb09 corpus to Freebase. We use global co-occurrence statistics between textual and knowledge base relations as the supervision signal to train the embedding. Evaluation on two relational understanding tasks demonstrates the usefulness of the learned textual relation embedding. The data and code can be found at https://github.com/czyssrs/GloREPlus

==> 05-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
 We introduce a new type of pre-trained embedding to represent textual relations. To solicit global co-occurrence frequencies as supervision signal from large open-domain corpus, we create the largest distant supervision dataset by linking the entire English ClueWeb09 to Freebase. Experiments on relation extraction and KB completion demonstrate that the learned embedding provides good prior knowledge to boost model performance, as well as alleviates the demands for designing task-specific textual relation models. 
%  The intrinsic evaluation result demonstrates the rich relational semantics encoded in the learned embeddings. This further indicates the embedding could potentially help unsupervised tasks in a more practical setting, where relational understanding is needed but labeled data are scarce. 
% The intrinsic analysis further indicates the embedding could potentially help unsupervised tasks in a more practical setting, where relational understanding is needed but labeled data are scarce. 




